Improving Cross-lingual Speech Synthesis with Triplet Training Scheme

Recent advances in cross-lingual text-to-speech (TTS) made it possible to synthesize speech in a language foreign to a monolingual speaker. However, there is still a large gap between the pronunciation of generated cross-lingual speech and that of native speakers in terms of naturalness and intelligibility. In this paper, a triplet training scheme is proposed to enhance the cross-lingual pronunciation by allowing previously unseen content and speaker combinations to be seen during training. Proposed method introduces an extra fine-tune stage with triplet loss during training, which efficiently draws the pronunciation of the synthesized foreign speech closer to those from the native anchor speaker, while preserving the non-native speaker's timbre. Experiments are conducted based on a state-of-the-art baseline cross-lingual TTS system and its enhanced variants. All the objective and subjective evaluations show the proposed method brings significant improvement in both intelligibility and naturalness of the synthesized cross-lingual speech.

==> backup <==

\begin{table*}[]
\label{spk2_2}
\centering
\caption{WER/CER of the synthesized cross-lingual speech with Expert Transfer (2-speaker dataset)}

\begin{tabular}{@{}ccccc@{}}
\toprule
Utterances                & Model                                     & Expert Transfer        & Mandarin   Speaker & English Speaker \\ \midrule
\multirow{9}{*}{Mandarin} & \multirow{5}{*}{Base-f0-energy}           & /                      & 0.081408           & 0.148413        \\
                          &                                           & Expert Dur             & /                  & 0.189655        \\
                          &                                           & Expert F0              & /                  & 0.139416        \\
                          &                                           & Expert Energy          & /                  & 0.170557        \\
                          &                                           & Expert   Dur/F0/Energy & /                  & 0.130281        \\ \cmidrule(l){2-5} 
                          & \multirow{4}{*}{Base-f0-energy + Triplet} & Expert Dur             & \textbf{0.073782}           & 0.162555        \\
                          &                                           & Expert F0              & 0.075385           & \textbf{0.114852}        \\
                          &                                           & Expert Energy          & 0.075519           & 0.159582        \\
                          &                                           & Expert   Dur/F0/Energy & 0.075727           & 0.125113        \\ \midrule
\multirow{9}{*}{English}  & \multirow{5}{*}{Base-f0-energy}           & /                      & 0.305865           & 0.182839        \\
                          &                                           & Expert Dur             & 0.252481           & /               \\
                          &                                           & Expert F0              & 0.260933           & /               \\
                          &                                           & Expert Energy          & 0.234825           & /               \\
                          &                                           & Expert   Dur/F0/Energy & \textbf{0.233302}           & /               \\ \cmidrule(l){2-5} 
                          & \multirow{4}{*}{Base-f0-energy + Triplet} & Expert Dur             & 0.2879             & \textbf{0.178789}        \\
                          &                                           & Expert F0              & 0.261638           & 0.181566        \\
                          &                                           & Expert Energy          & 0.257              & 0.183379        \\
                          &                                           & Expert   Dur/F0/Energy & 0.257487           & 0.18035         \\ \bottomrule
\end{tabular}

\end{table*}





\begin{table}[]
\label{spk2_1}
\centering
\caption{WER/CER of the synthesized cross-lingual speech (2-speaker dataset)}
\begin{tabular}{@{}cccc@{}}
\toprule
Utterances                & Model          & Mandarin   Speaker & English Speaker   \\ \midrule
\multirow{2}{*}{Mandarin} & Base           & \textbf{0.072797}  & 0.151192          \\
                          & Base + Triplet & 0.082452           & \textbf{0.11319}  \\ \midrule
\multirow{2}{*}{English}  & Base           & 0.29784            & \textbf{0.186606} \\
                          & Base + Triplet & \textbf{0.280365}  & 0.189684          \\ \bottomrule
\end{tabular}
\end{table}






% 3spk

\begin{tabular}{@{}lllll@{}}
\toprule
Utterances                & Model                                     & Expert Transfer        & Mandarin   Speaker & English Speaker   \\ \midrule
\multirow{9}{*}{Mandarin} & \multirow{5}{*}{Base-f0-energy}           & /                      & \textbf{0.073673}  & 0.148413          \\
                          &                                           & Expert Dur             & /                  & 0.160735          \\
                          &                                           & Expert F0              & /                  & 0.106274          \\
                          &                                           & Expert Energy          & /                  & 0.150404          \\
                          &                                           & Expert   Dur/F0/Energy & /                  & 0.108847          \\ \cmidrule(l){2-5} 
                          & \multirow{4}{*}{Base-f0-energy + Triplet} & Expert Dur             & TODO(9.15)               & TODO(9.15)              \\
                          &                                           & Expert F0              & TODO(9.15)               & TODO(9.15)              \\
                          &                                           & Expert Energy          & TODO(9.15)               & TODO(9.15)              \\
                          &                                           & Expert   Dur/F0/Energy & 0.076413           & \textbf{0.095399} \\ \cmidrule(l){2-5} 
\multirow{9}{*}{English}  & \multirow{5}{*}{Base-f0-energy}           & /                      & 0.305865           & \textbf{0.17887}  \\
                          &                                           & Expert Dur             & 0.295165           & /                 \\
                          &                                           & Expert F0              & 0.296497           & /                 \\
                          &                                           & Expert Energy          & 0.304394           & /                 \\
                          &                                           & Expert   Dur/F0/Energy & 0.300355           & /                 \\ \cmidrule(l){2-5} 
                          & \multirow{4}{*}{Base-f0-energy + Triplet} & Expert Dur             & TODO (9.15)              & TODO(9.15)              \\
                          &                                           & Expert F0              & TODO(9.15)               & TODO(9.15)              \\
                          &                                           & Expert Energy          & TODO (9.15)              & TODO(9.15)              \\
                          &                                           & Expert   Dur/F0/Energy & \textbf{0.277071}  & 0.180972          \\ \bottomrule
\end{tabular}


%%%%%%%%%%%%%%% wer with punctuations %%%%%%%%%%%%%
Object Metrics:

\begin{table}[h]
\label{spk3_1}
\centering
\caption{WER/CER of the synthesized cross-lingual speech without native speaker embedding transfer.}
\begin{tabular}{@{}cccccc@{}}
\toprule
                                                          & \multicolumn{3}{c}{English Utterances}                                                                                                                                                     & \multicolumn{2}{c}{Mandarin Utterances}                                                                                    \\ \midrule
Model                                                     & \begin{tabular}[c]{@{}c@{}}English \\ Speaker\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mandarin \\ Speaker-M\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mandarin \\ Speaker-F\end{tabular} & \begin{tabular}[c]{@{}c@{}}English \\ Speaker\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mandarin \\ Speaker-F\end{tabular} \\ \midrule
Base                                                      & 0.187437                                                   & 0.318447                                                      & 0.319932                                                      & 0.147836                                                   & 0.078043                                                      \\
\begin{tabular}[c]{@{}c@{}}Base \\ + Triplet\end{tabular} & \textbf{0.185647}                                          & \textbf{0.261958}                                             & \textbf{0.276088}                                             & \textbf{0.114567}                                          & \textbf{0.073077}                                             \\ \bottomrule
\end{tabular}
\end{table}


\begin{table*}[h]
\label{spk3_2}
\centering
\caption{WER/CER of the synthesized cross-lingual speech with native speaker embedding transfer.}

\begin{tabular}{ccccccccc}
\hline
                                                                       &                                                                            &                                                                                                    &                                                                               & \multicolumn{3}{c}{English Utterances}                                                                                                                                                    & \multicolumn{2}{c}{Mandarin Utterances}                                                                                   \\ \hline
Model                                                                  & \begin{tabular}[c]{@{}c@{}}Dur-Native \\ Speaker \\ Embedding\end{tabular} & \begin{tabular}[c]{@{}c@{}}F0-Native \\ Speaker \\ Embedding \\ + Linear \\ Transform\end{tabular} & \begin{tabular}[c]{@{}c@{}}Energy-Native \\ Speaker \\ Embedding\end{tabular} & \begin{tabular}[c]{@{}c@{}}English \\ Speaker\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mandarin \\ Speaker-M\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mandarin\\ Speaker-F\end{tabular} & \begin{tabular}[c]{@{}c@{}}English\\ Speaker\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mandarin \\ Speaker-F\end{tabular} \\ \hline
\multirow{5}{*}{Base-f0-energy}                                        & NO                                                                         & NO                                                                                                 & NO                                                                            & \textbf{0.17887}                                           & 0.319509                                                      & 0.305865                                                     & 0.148413                                                  & 0.073673                                                      \\
                                                                       & YES                                                                        & NO                                                                                                 & NO                                                                            & /                                                          & 0.316194                                                      & 0.295165                                                     & 0.160735                                                  & /                                                             \\
                                                                       & NO                                                                         & YES                                                                                                & NO                                                                            & /                                                          & 0.306107                                                      & 0.296497                                                     & 0.106274                                                  & /                                                             \\
                                                                       & NO                                                                         & NO                                                                                                 & YES                                                                           & /                                                          & 0.288328                                                      & 0.304394                                                     & 0.150404                                                  & /                                                             \\
                                                                       & YES                                                                        & YES                                                                                                & YES                                                                           & /                                                          & 0.275097                                                      & 0.300355                                                     & 0.108847                                                  & /                                                             \\ \hline
\begin{tabular}[c]{@{}c@{}}Base-f0-energy  \\ + Triplet A\end{tabular} & NO                                                                         & NO                                                                                                 & NO                                                                            & 0.185860                                                   & 0.281759                                                      & 0.257575                                                     & 0.124673                                                  & \textbf{0.072286}                                             \\
\begin{tabular}[c]{@{}c@{}}Base-f0-energy  \\ + Triplet B\end{tabular} & YES                                                                        & NO                                                                                                 & NO                                                                            & 0.188882                                                   & 0.273211                                                      & \textbf{0.254927}                                            & 0.108724                                                  & 0.074917                                                      \\
\begin{tabular}[c]{@{}c@{}}Base-f0-energy\\  + Triplet C\end{tabular}  & NO                                                                         & YES                                                                                                & NO                                                                            & 0.191420                                                   & 0.277482                                                      & 0.272903                                                     & 0.143829                                                  & 0.076146                                                      \\
\begin{tabular}[c]{@{}c@{}}Base-f0-energy  \\ + Triplet D\end{tabular} & NO                                                                         & NO                                                                                                 & YES                                                                           & 0.180785                                                   & \textbf{0.258999}                                             & 0.257199                                                     & 0.155668                                                  & 0.074921                                                      \\
\begin{tabular}[c]{@{}c@{}}Base-f0-energy \\ + Triplet E\end{tabular}  & YES                                                                        & YES                                                                                                & YES                                                                           & 0.180972                                                   & 0.27308                                                       & 0.277071                                                     & \textbf{0.095399}                                         & 0.076413                                                      \\ \hline
\end{tabular}

\end{table*}







\begin{table*}[h]
\addtolength{\tabcolsep}{-2pt}
\label{spk3_2}
\centering
\caption{WER/CER of the synthesized cross-lingual speech with native speaker embedding transfer.}

\begin{tabular}{ccccccccccc}
\hline
                                                                       &                                                                            &                                                                                                    &                                                                               & \multicolumn{3}{c}{English Utterances}                                                                                                                                                    &  & \multicolumn{2}{c}{Mandarin Utterances}                                                                                   &                \\ \cline{5-7} \cline{9-10}
Model                                                                  & \begin{tabular}[c]{@{}c@{}}Dur-Native \\ Speaker \\ Embedding\end{tabular} & \begin{tabular}[c]{@{}c@{}}F0-Native \\ Speaker \\ Embedding \\ + Linear \\ Transform\end{tabular} & \begin{tabular}[c]{@{}c@{}}Energy-Native \\ Speaker \\ Embedding\end{tabular} & \begin{tabular}[c]{@{}c@{}}English \\ Speaker\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mandarin \\ Speaker-M\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mandarin\\ Speaker-F\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}English\\ Speaker\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mandarin \\ Speaker-F\end{tabular} & Average        \\ \hline
\multirow{5}{*}{Base-f0-energy}                                        & NO                                                                         & NO                                                                                                 & NO                                                                            & \textbf{0.112}                                             & 0.243                                                         & 0.261                                                        &  & 0.134                                                     & \textbf{0.049}                                                & 0.160          \\
                                                                       & YES                                                                        & NO                                                                                                 & NO                                                                            & /                                                          & 0.238                                                         & 0.252                                                        &  & 0.143                                                     & /                                                             & 0.159          \\
                                                                       & NO                                                                         & YES                                                                                                & NO                                                                            & /                                                          & \textbf{0.237}                                                & 0.247                                                        &  & \textbf{0.084}                                            & /                                                             & 0.146          \\
                                                                       & NO                                                                         & NO                                                                                                 & YES                                                                           & /                                                          & 0.245                                                         & 0.232                                                        &  & 0.137                                                     & /                                                             & 0.155          \\
                                                                       & YES                                                                        & YES                                                                                                & YES                                                                           & /                                                          & 0.244                                                         & \textbf{0.213}                                               &  & 0.086                                                     & /                                                             & \textbf{0.141} \\ \hline
\begin{tabular}[c]{@{}c@{}}Base-f0-energy  \\ + Triplet A\end{tabular} & NO                                                                         & NO                                                                                                 & NO                                                                            & 0.119                                                      & 0.197                                                         & 0.218                                                        &  & 0.107                                                     & \textbf{0.049}                                                & 0.138          \\
\begin{tabular}[c]{@{}c@{}}Base-f0-energy  \\ + Triplet B\end{tabular} & YES                                                                        & NO                                                                                                 & NO                                                                            & 0.120                                                      & \textbf{0.192}                                                & 0.207                                                        &  & 0.143                                                     & 0.050                                                         & 0.142          \\
\begin{tabular}[c]{@{}c@{}}Base-f0-energy\\  + Triplet C\end{tabular}  & NO                                                                         & YES                                                                                                & NO                                                                            & 0.123                                                      & 0.209                                                         & 0.214                                                        &  & 0.090                                                     & 0.052                                                         & 0.138          \\
\begin{tabular}[c]{@{}c@{}}Base-f0-energy  \\ + Triplet D\end{tabular} & NO                                                                         & NO                                                                                                 & YES                                                                           & 0.116                                                      & 0.196                                                         & \textbf{0.205}                                               &  & 0.128                                                     & 0.050                                                         & 0.139          \\
\begin{tabular}[c]{@{}c@{}}Base-f0-energy \\ + Triplet E\end{tabular}  & YES                                                                        & YES                                                                                                & YES                                                                           & \textbf{0.113}                                             & 0.219                                                         & 0.211                                                        &  & \textbf{0.075}                                            & 0.052                                                         & \textbf{0.134} \\ \hline
\end{tabular}

\end{table*}

- CER/WER (cross-lingual)



\begin{table}[h]

\centering
\caption{Systems built in experiments.}

\addtolength{\tabcolsep}{-5pt}

\begin{tabular}{|c|l|}
\hline
Systems                                                               & \multicolumn{1}{c|}{Details}                                                                                                        \\ \hline
Base                                                                  & DurIAN with IPA                                                                                                                     \\ \hline
Base + triplet                                                        & \begin{tabular}[c]{@{}l@{}}Base with triplet fine-tune\\  training\end{tabular}                                                     \\ \hline
Base-f0-energy                                                        & \begin{tabular}[c]{@{}l@{}}DurIAN with auxiliary f0 \\ and energy predictors\end{tabular}                                           \\ \hline
\begin{tabular}[c]{@{}c@{}}Base-f0-energy \\ + triplet A\end{tabular} & \begin{tabular}[c]{@{}l@{}}Base-f0-energy with triplet \\ fine-tune training\end{tabular}                                           \\ \hline
\begin{tabular}[c]{@{}c@{}}Base-f0-energy \\ + triplet B\end{tabular} & \begin{tabular}[c]{@{}l@{}}Base-f0-energy with triplet  \\ fine-tune  training with duration transferred.\end{tabular}              \\ \hline
\begin{tabular}[c]{@{}c@{}}Base-f0-energy \\ + triplet C\end{tabular} & \begin{tabular}[c]{@{}l@{}}Base-f0-energy with triplet \\ fine-tune  training with f0 transferred.\end{tabular}                     \\ \hline
\begin{tabular}[c]{@{}c@{}}Base-f0-energy \\ + triplet D\end{tabular} & \begin{tabular}[c]{@{}l@{}}Base-f0-energy with triplet \\ fine-tune  training with energy transferred.\end{tabular}                 \\ \hline
\begin{tabular}[c]{@{}c@{}}Base-f0-energy \\ + triplet E\end{tabular} & \begin{tabular}[c]{@{}l@{}}Base-f0-energy with triplet fine-tune  training\\ with f0, energy and duration transferred.\end{tabular} \\ \hline
\end{tabular}
\label{system_intro}
\end{table}





\begin{table}[]
\addtolength{\tabcolsep}{-3pt}
\centering
\caption{Triplets constructed for unseen combinations}
\begin{tabular}{|l|l|l|}
\hline
\multirow{2}{*}{Set 1} & CT & $t^C_i(M^{an}_{i, EN-SPK}, \hat{M}^{pos}_{i, CN-SPK-M}, None)$                  \\ \cline{2-3} 
                       & ST & $t^S_i(M^{an}_{i, CN-SPK-M}, \hat{M}^{pos}_{i, CN-SPK-M}, M^{neg}_{i, EN-SPK})$ \\ \hline
\multirow{2}{*}{Set 2} & CT & $t^C_i(M^{an}_{i, EN-SPK}, \hat{M}^{pos}_{i, CN-SPK-F}, None)$                  \\ \cline{2-3} 
                       & ST & $t^S_i(M^{an}_{i, CN-SPK-F}, \hat{M}^{pos}_{i, CN-SPK-F}, M^{neg}_{i, EN-SPK})$ \\ \hline
\multirow{2}{*}{Set 3} & CT & $t^C_i(M^{an}_{i, CN-SPK-M}, \hat{M}^{pos}_{i, EN-SPK}, None)$                  \\ \cline{2-3} 
                       & ST & $t^S_i(M^{an}_{i, EN-SPK}, \hat{M}^{pos}_{i, EN-SPK}, M^{neg}_{i, CN-SPK-F})$   \\ \hline
\end{tabular}
\label{triplets_exp}
\end{table}





\begin{tabular}{ccccccccccc}
\hline
                                &                                                                            &                                                                                                    &                                                                               & \multicolumn{3}{c}{EN target}                                                                                                                                 &  & \multicolumn{2}{c}{CN target}                                                                           &                \\ \cline{5-7} \cline{9-10}
System                           & \begin{tabular}[c]{@{}c@{}}Dur-transfer\end{tabular} & \begin{tabular}[c]{@{}c@{}}F0-transfer\end{tabular} & \begin{tabular}[c]{@{}c@{}}Energy-transfer\end{tabular} & \begin{tabular}[c]{@{}c@{}}EN- \\ SPK\end{tabular} & \begin{tabular}[c]{@{}c@{}}CN- \\ SPK-M\end{tabular} & \begin{tabular}[c]{@{}c@{}}CN- \\ SPK-F\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}EN- \\ SPK\end{tabular} & \begin{tabular}[c]{@{}c@{}}CN- \\ SPK-F\end{tabular} & Average        \\ \hline
\multirow{5}{*}{Base-FE} & NO                                                                         & NO                                                                                                 & NO                                                                            & \textbf{0.112}                                    & 0.243                                               & 0.261                                               &  & 0.134                                             & \textbf{0.049}                                      & 0.160          \\
                                & YES                                                                        & NO                                                                                                 & NO                                                                            & /                                                 & 0.238                                               & 0.252                                               &  & 0.143                                             & /                                                   & 0.159          \\
                                & NO                                                                         & YES                                                                                                & NO                                                                            & /                                                 & \textbf{0.237}                                      & 0.247                                               &  & \textbf{0.084}                                    & /                                                   & 0.146          \\
                                & NO                                                                         & NO                                                                                                 & YES                                                                           & /                                                 & 0.245                                               & 0.232                                               &  & 0.137                                             & /                                                   & 0.155          \\
                                & YES                                                                        & YES                                                                                                & YES                                                                           & /                                                 & 0.244                                               & \textbf{0.213}                                      &  & 0.086                                             & /                                                   & \textbf{0.141} \\ \hline
Base-FE  + Triplet A     & NO                                                                         & NO                                                                                                 & NO                                                                            & 0.119                                             & 0.197                                               & 0.218                                               &  & 0.107                                             & \textbf{0.049}                                      & 0.138          \\
Base-FE  + Triplet B     & YES                                                                        & NO                                                                                                 & NO                                                                            & 0.120                                             & \textbf{0.192}                                      & 0.207                                               &  & 0.143                                             & 0.050                                               & 0.142          \\
Base-FE + Triplet C      & NO                                                                         & YES                                                                                                & NO                                                                            & 0.123                                             & 0.209                                               & 0.214                                               &  & 0.090                                             & 0.052                                               & 0.138          \\
Base-FE  + Triplet D     & NO                                                                         & NO                                                                                                 & YES                                                                           & 0.116                                             & 0.196                                               & \textbf{0.205}                                      &  & 0.128                                             & 0.050                                               & 0.139          \\
Base-FE + Triplet E      & YES                                                                        & YES                                                                                                & YES                                                                           & \textbf{0.113}                                    & 0.219                                               & 0.211                                               &  & \textbf{0.075}                                    & 0.052                                               & \textbf{0.134} \\ \hline
\end{tabular}



\begin{tabular}{ccclcccccccc}
\hline
                                                                      & EN utterance          & CN utterance   &  & \multicolumn{5}{c}{EN utterance}                                                        &  & \multicolumn{2}{c}{CN utterance}           \\ \cline{2-3} \cline{5-9} \cline{11-12} 
Speakers                                                              & EN SPK             & CN SPK-F    &  & \multicolumn{2}{c}{CN SPK-M}            &  & \multicolumn{2}{c}{CN SPK-F}            &  & \multicolumn{2}{c}{EN SPK}              \\ \cline{2-3} \cline{5-6} \cline{8-9} \cline{11-12} 
System                                                                & Naturalness        & Naturalness &  & Naturalness        & Similarity         &  & Naturalness        & Similarity         &  & Naturalness        & Similarity         \\ \hline
Base                                                                  & 3.28±0.66          & 4.19±0.46   &  & 2.98±0.63          & 3.33±0.75          &  & 3.15±0.76          & 3.40±0.53          &  & 2.73±0.67          & 3.31±0.93          \\
Base + Triplet                                                        & 3.57±0.51          & 4.29±0.37   &  & 3.31±0.59          & 3.60±0.90          &  & 3.35±0.76          & 3.64±0.74          &  & 2.99±0.63          & 3.58±0.49          \\
Base-FE                                                        & 3.98±0.46          & \textbf{4.33±0.35}   &  & \textbf{3.33±0.76} & 3.58±0.69          &  & 3.39±0.60          & 3.56±0.78          &  & 3.20±0.50          & 3.56±0.77          \\
\begin{tabular}[c]{@{}c@{}}Base-FE \\ + Triplet E\end{tabular} & \textbf{3.99±0.47} & 4.26±0.42   &  & 3.21±0.69          & \textbf{3.60±0.55} &  & \textbf{3.59±0.47} & \textbf{3.82±0.55} &  & \textbf{3.36±0.39} & \textbf{3.77±0.37} \\ \hline
Ground Truth                                                          & 4.39±0.21          & 4.46±0.13   &  & /                  & /                  &  & /                  & /                  &  & /                  & /                  \\ \hline
\end{tabular}




\begin{tabular}{ccclcccccccc}
\hline
                                                                      & EN utterance          & CN utterance   &  & \multicolumn{5}{c}{EN utterance}                                                        &  & \multicolumn{2}{c}{CN utterance}           \\ \cline{2-3} \cline{5-9} \cline{11-12} 
Speakers                                                              & EN-SPK             & CN-SPK-F    &  & \multicolumn{2}{c}{CN-SPK-M}            &  & \multicolumn{2}{c}{CN-SPK-F}            &  & \multicolumn{2}{c}{EN-SPK}              \\ \cline{2-3} \cline{5-6} \cline{8-9} \cline{11-12} 
System                                                                & Naturalness        & Naturalness &  & Naturalness        & Similarity         &  & Naturalness        & Similarity         &  & Naturalness        & Similarity         \\ \hline
Base                                                                  & 3.28±0.66          & 4.19±0.46   &  & 2.98±0.63          & 3.33±0.75          &  & 3.15±0.76          & 3.40±0.53          &  & 2.73±0.67          & 3.31±0.93          \\
+ Triplet                                                       & 3.57±0.51          & 4.29±0.37   &  & 3.31±0.59          & 3.60±0.90          &  & 3.35±0.76          & 3.64±0.74          &  & 2.99±0.63          & 3.58±0.49          \\
Base-FE                                                        & 3.98±0.46          & \textbf{4.33±0.35}   &  & \textbf{3.33±0.76} & 3.58±0.69          &  & 3.39±0.60          & 3.56±0.78          &  & 3.20±0.50          & 3.56±0.77          \\
\begin{tabular}[c]{@{}c@{}} + Triplet-DFE\end{tabular} & \textbf{3.99±0.47} & 4.26±0.42   &  & 3.21±0.69          & \textbf{3.60±0.55} &  & \textbf{3.59±0.47} & \textbf{3.82±0.55} &  & \textbf{3.36±0.39} & \textbf{3.77±0.37} \\ \hline
Ground Truth                                                          & 4.39±0.21          & 4.46±0.13   &  & /                  & /                  &  & /                  & /                  &  & /                  & /                  \\ \hline
\end{tabular}


\begin{table}[t]
\vspace{-10pt}
\addtolength{\tabcolsep}{-5pt}
\small
\centering
\caption{WER evaluation on intelligibility with prosody features transfer based on Base-FE.}

\begin{tabular}{ccccccccccc}
\hline
                         &    &    &    & \multicolumn{3}{c}{EN utterance}                                                                                                                                 &  & \multicolumn{2}{c}{CN utterance}                                                                           &                \\ \cline{5-7} \cline{9-10}
System                    & D* & F* & E* & \begin{tabular}[c]{@{}c@{}}EN-\\SPK\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textit{CN-}}\\\textbf{\textit{SPK-M}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textit{CN-}}\\\textbf{\textit{SPK-F}}\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}\textbf{\textit{EN-}}\\\textbf{\textit{SPK}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}CN-\\SPK-F\end{tabular} & AVG            \\ \hline
\multirow{5}{*}{Base-FE} & N  & N  & N  & \textbf{0.112}                                    & 0.243                                               & 0.261                                               &  & 0.134                                             & \textbf{0.049}                                      & 0.160          \\
                         & Y  & N  & N  & /                                                 & 0.238                                               & 0.252                                               &  & 0.143                                             & /                                                   & 0.159          \\
                         & N  & Y  & N  & /                                                 & \textbf{0.237}                                      & 0.247                                               &  & \textbf{0.084}                                    & /                                                   & 0.146          \\
                         & N  & N  & Y  & /                                                 & 0.245                                               & 0.232                                               &  & 0.137                                             & /                                                   & 0.155          \\
                         & Y  & Y  & Y  & /                                                 & 0.244                                               & \textbf{0.213}                                      &  & 0.086                                             & /                                                   & \textbf{0.141} \\ \hline
+ Triplet              & N  & N  & N  & 0.119                                             & 0.197                                               & 0.218                                               &  & 0.107                                             & \textbf{0.049}                                      & 0.138          \\
+ Triplet-D              & Y  & N  & N  & 0.120                                             & \textbf{0.192}                                      & 0.207                                               &  & 0.143                                             & 0.050                                               & 0.142          \\
+ Triplet-F              & N  & Y  & N  & 0.123                                             & 0.209                                               & 0.214                                               &  & 0.090                                             & 0.052                                               & 0.138          \\
+ Triplet-E              & N  & N  & Y  & 0.116                                             & 0.196                                               & \textbf{0.205}                                      &  & 0.128                                             & 0.050                                               & 0.139          \\
+ Triplet-DFE              & Y  & Y  & Y  & \textbf{0.113}                                    & 0.219                                               & 0.211                                               &  & \textbf{0.075}                                    & 0.052                                               & \textbf{0.134} \\ \hline
\end{tabular}
\begin{tablenotes}
\textit{D*}, \textit{F*}, \textit{E*} represent duration, f0, energy transfer respectively in inference for inter-lan tests.
\end{tablenotes}
\label{spk3_2}
\vspace{-10pt}
\end{table}
